Reduction of transient noise artifacts in gravitational-wave data using deep learning

Excess transient noise artifacts, or glitches impact the data quality of ground-based gravitational-wave (GW) detectors and impair the detection of signals produced by astrophysical sources. Mitigation of glitches is crucial for improving GW signal detectability. However, glitches are the product of short-lived linear and non-linear couplings among the interrelated detector-control systems that include optic alignment systems and mitigation of seismic disturbances, generally making it difficult to model noise couplings. Hence, typically time periods containing glitches are vetoed to mitigate the effect of glitches in GW searches at the cost of reduction of the analyzable data. To increase the available data period and improve the detectability for both model and unmodeled GW signals, we present a new machine learning based method which uses on-site sensors/system-controls monitoring the instrumental and environmental conditions to model noise couplings and subtract glitches in GW detector data. We find that our method reduces 20-70% of the excess power in the data due to glitches. By injecting software simulated signals into the data and recovering them with one of the unmodeled GW detection pipelines, we address the robustness of the glitch-reduction technique to efficiently remove glitches with no unintended effects on GW signals.

==> discussion_conclusion.tex <==
\section{Conclusion} \label{ppr2_conclusion}
In this paper, we have presented a new machine learning-based algorithm to subtract glitches using a set of auxiliary channels. Glitches are the product of short-live linear and non-linear couplings due to interrelated sub-systems in the detector including the optic alignment systems and mitigation systems of ground motions. Because of the characteristic of glitches, modeling coupling mechanisms is typically challenging. Without the prior knowledge of the physical coupling mechanisms, our algorithm takes the data from the sensors monitoring the instrumental and environmental noise transients and then estimates the glitch waveform in the detector's output, providing the glitch-subtracted data stream. Subtraction of glitches significantly improves the quality of the data and will enhance the detectability of astrophysical \ac{GW} signals. 

Using two classes of glitches with distinct noise couplings in the \ac{aLIGO} data, we find that our algorithm successfully reduces the \ac{SNR} of the data due to the presence of glitches by $10-70$\%. Reduction of energy due to the presence of glitches in the data enhances the ranking statistic of one of the \ac{GW} unmodeled signal detection pipelines called \ac{cWB} up to $\sim 800$\% without introducing unintended effects on astrophysical signals.

We find that using the spectrograms of the data as the input for the network is more successful than using time series as the input. However, it might improve the glitch subtraction efficiency by using the Griffin-Lim transformation as well as the amplitude and phase corrections within the loss function to train the network. Improved glitch subtraction would allow us to detect astrophysical signals with higher confidence and brings us a better understanding of the physics in the universe.     






==> introduction.tex <==
\section{Introduction} \label{intro}

% current GW detections, what needs
The first detection of a gravitational-wave (\ac{GW}) signal from a \ac{BBH} merger \cite{Abbott:2016GW150914} on September 14th, 2015 was the breakthrough of \ac{GW} astronomy. Since then, about 50 high confidence detections \cite{GWTC-1, Abbott:2020niy, LIGOScientific:2020stg, PhysRevLett.125.101102, Abbott_2020, Abbott:2020khf} have been made by the network of \ac{GW} detectors currently consisting of the two LIGO detectors in the United States \cite{advLigo2015}, the Virgo detector in Italy \cite{advVirgo2015}, the GEO-HF detector in Germany \cite{Luck:2010rt}, the KAGRA detector in Japan \cite{Akutsu:2020his}, and eventually the LIGO-India in India \cite{LIGO-India}. One of the dominating factors for the breakthough in 2015 was the improvement of the detector sensitivity by a factor of $\sim 10$ at the detector's most sensitive frequency compared to the initial LIGO \cite{advLigo2015}. Reducing transient and periodic noise sources in instrumental and environmental origin may enhance the identification of \ac{GW} signals by increasing the significance of candidate events of astrophysical signals and avoiding classifying them as sub-threshold triggers \cite{GWTC-1, Riles:2012yw}. 

% instrument subsystem 
% introduction of many sensors 
% concept of the witness channels 

The physical couplings due to the detector design are noise sources such as the fluctuating amplitude of laser light in the arm cavities, fluctuations of the photon arrival time at the output-port photodiode, thermal fluctuations of mirror coatings, and optic suspension \cite{TheLIGOScientific:2014jea}. Besides, during observation runs, environmental and instrumental noise sources including wind or ground motions as well as optic-controlling systems limit the detector sensitivity \cite{TheLIGOScientific:2016zmo}. Reducing the effect of these noise sources on the detector's output, \textit{strain} channel, is crucial to improve the detectability of any \ac{GW} signals and better understand physics in the universe. 

The \ac{aLIGO} detector use approximately two hundred thousands auxiliary \textit{channels} such as sensors/control-systems reading-out environmental or instrumental conditions inside and around detectors in parallel to the detector's output readout in time domain. These auxiliary channels can be potential witnesses of couplings of noise sources and can be used to subtract the noise in the strain channel.

% subtraction method for long-lasting noise 
Long-lasting noise sources with a duration longer than $\sim 4$ seconds have linear and/or non-linear non-stationary coupling mechanisms (Ref. \cite{Ormiston:2020ele} set the analysis window to be 8 seconds for the long-lasting noise). Among others, the main technique to subtract linearly coupled long-lasting noise sources is to calculate coherence between the witness channels and the strain channel. For example, the main source in $\sim50-1000$ Hz frequency band coupled linearly with the jitter of the pre-stabilization laser beam in angle and size was subtracted \cite{Driggers:2018gii, Kwee:12, Robert:2016gii, Davis:2018yrz}. For non-linearly and non-stationary coupled noise sources in environmental and instrumental origin, techniques with machine learning algorithms show successful subtractions and improve the detector sensitivity \cite{Tiwari:2015ofa, Meadors:2013lja, Mukund:2020lby, Vajente:2019ycy, Ormiston:2020ele}. 

% GW detectors are very susceptible to glitches
% ---> because glitches may resemble astrophysical signals 
% why it matters
% ----> reduce confidence in the significance of GW candidates
% why not subtract them? 
% ----> they are complicated (problem statement)
% current solutions (current infrastructures) 
% ---- > just veto them based on coincidence tests (current infrastructure)

Other than long-lasting noise, transient noise artifacts, or \textit{glitches} significantly impair the quality of \ac{GW} detector data and reduce confidence in the significance of candidate \ac{GW} events because glitches may resemble astrophysical signals. Glitch removal is crucial for \ac{GW} signal searches. However, glitches are the product of \textbf{short-lived} linear and non-linear couplings among interrelated detector subsystems, generally making it difficult to find their coupling mechanisms. To mitigate the effect of glitches on \ac{GW} searches, LIGO-Virgo collaboration vetoes time periods where glitches are present \cite{Davis:2021ecd, Abbott:2020niy} or reduces the significance of \ac{GW} candidates based on the probability of the glitch presence \cite{Godwin:2020weu}. Software engines such as \ac{UPV} \cite{Isogai:2010zz(UPV)}, \ac{hVETO} \cite{Smith:2011an(hVETO)}, Pointy Poisson \cite{Essick:2020cyv}, PyChChoo \cite{mogushi2021application}, and \textsc{iDQ} \cite{Biswas:2013wfa, Essick:2020qpo} find the statistical correlation of glitches between the detector's output and numerous auxiliary channels to identify the presence of glitches while avoiding the mitigation of astrophysical signals. 

The above mitigation techniques have disadvantages: reduction of the analyzable data which might contain \ac{GW} signals or reduction of the significance of \ac{GW} signal candidates. Therefore, it is desirable to subtract glitches for overcoming the above disadvantages. The functional forms to model the coupling mechanisms of glitches can require detailed knowledge of instrumental subsystems and a large number of parameters \cite{Was:2020ziy}. Also, there exist situations where functional forms can not be obtained because of unknown physical mechanisms about glitches. In addition to subtraction techniques for long-lasting noise sources noted above, other machine learning techniques have shown promising applications to \ac{GW} astronomy \cite{Cuoco:2020ogp}. For example, the classification of glitches helps scientists characterize data \cite{Zevin:2016qwy, Soni:2021cjy, Mukund:2016thr}, the technique characterizes glitches based on auxiliary channels \cite{Biswas:2013wfa}, and the method removes the effect of a glitch in coincidence with a signal produced from \ac{CBC} mergers \cite{Mogushi:2021cpw}. These successes motivate us to develop a new machine learning-based method to subtract glitches using auxiliary channels with no dependency from any astrophysical signal waveforms and no precise prior knowledge of all the system configurations, allowing the method to be easily adaptive to changes in the detector settings.

% [new solution]
% our paper 
In this paper, we present a machine learning-based algorithm that uses auxiliary witness channels to subtract glitches in the detector's output. Using two classes of glitches that are adversely affecting unmodeled \ac{GW} detection searches \cite{mogushi2021application}, we characterize the performance of our subtraction technique. Adding simulated \ac{GW} signals to the data before subtraction, we validate the algorithm not to manipulate or introduce biases to the resultant estimates of the astrophysical parameters.  



